Subgroups of a free group with every growth rate

For every $\alpha \in [1,2r-1]$, we show there exists a subgroup $H<F_r$ whose growth rate is $\alpha$.

==> tmp.tex <==
\section{A new approach}
\ML{this is me}
Ok maybe I am wrong, but let's try this.

Our goal is to construct a random graph whose universal cover is the Galton Watson tree with offspring distribution given by some $P\sim \text{Poisson }(\lambda)$, for any $\lambda>1$. We also need for this graph to have at least one circle. 


We will define this graph inductively. The vertices of the graph will be the set of natural numbers $\N$.  At each step $n$, connect the $n-$th vertex with the numbers in $[n-1]$ independently with probability $\lambda/n$ ( for $n$ large enough of course). Call the resulting graph $G$.

Notice that for every fixed $k$, the number of neighbors of $k$ will be given by a Poisson $(\lambda)$ random variable since
\begin{align}\label{neighb}
    N_k= \sum_{l=1}^{k-1}X_{l,k}+ \sum_{l=k+1}^{\infty} X_{l,k}
\end{align}
where $X_{i,k}$ is a Bernoulli random variable with probability of success $\lambda/\max\{j,k\}$.  The Poisson limit theorem states that for every sequence of Bernoulli's such that $np_n\to \lambda$, the sum of the Bernoulli will converge to the poisson law. Thusm it is ensured that \eqref{neighb} is a Poisson.  Notice that this allows us to exclude any finite number of neighbors of a vertex and still get a Poisson law ( thus a non-backtracking walk would not affect the distribution). Two issues
\begin{itemize}
    \item I think we can prove that the graph has circles. ( I believe that the number of triangles when the vertices are $n$ should be something like $\log n$)
    \item In the definition of the Galton Watson tree, you have complete independence. For this I suppose we can have some smart coupling. We will see.
\end{itemize}
This model is named Barak-Erdős in the bibliography but it is either assumed to be finite or directed.

We have an issue with this model, the degree is not bounded. 


\section{Another try}
Take the assumptions of Lemma \ref{lemma:convergence_subgraphs} and add the following two Assumption
\begin{itemize}
    \item For each graph $G_n$ there exists a large constant $m_n(=\delta_0\log_{a-\epsilon_n}k(n), $ appropriate sequence $k(n)$ in order for the convergence to hold), for which it is true that  
    \begin{align}\label{bound_norm_non_back}
        \| B_{G_n}^{m_n}\|\leq  2a(G_n)^{m_n} (\text{ here 2 can be replaced by any absolute constant C we will see})
    \end{align}
    The sequence $m_n$ is increasing and goes to infinity.
    \item Partition the set of natural numbers into the set $\mathbb{N}=\cup_{r=1}^{\infty}[m_r,m_{r+1})\cup [1,m_1)$. Assume that  there exists a vertex $v_0 \in V(G_0)$ such that for any $r\geq m_1$ if $r \in [m_l,m_{l+1})$, then the $r$-neighborhood of $v_0$ in $G$ does not contain vertices which belong to $\cup_{x=l+1}^{\infty} V(G_x)$
\end{itemize}
Set $NB_{m}(v_0)$ to be the set of \textbf{closed} non backtracking walks of $G$ of length $m$ starting and ending in $v_0$. Let $t \in \N$ large. Suppose $t \in [m_r,m_{r+1})$ for some $r$. Then 
\begin{align}
   & |NB_{t}(v_0)|=|\text{non backtracking closed walks starting and ending in }v_0 \text{ inside the graph } G_r|\\&\leq \|B_{G_r}^{t}\|\leq 2^{t/m_r}a(G_n)^{r}  \leq 2^{t/m_r} a^{r}_0
\end{align}
Thus we get that
\begin{align}
  |NB_{t}(v_0)|^{1/t}\leq   2^{1/m_r}a_0
\end{align}
By picking $t$ large enough ( and thus $m_r$  being large) we get that $2^{1/m_r}\leq 1+\epsilon$ (for arbitrary small $\epsilon>0$). The claim follows. 
\section{our model}
Recall our result in \cite{louvaris2024density}. For each of the $H_k$ we have proven a bound for the norm of the non backtracking matrix, actually we applied Proposition 7 of \cite{bordenave2015non} which gives a bound to the spectral norm of the non backtracking matrix as the one in \eqref{bound_norm_non_back}.
ISSUES to see
\begin{itemize}
    \item Can we make the same bound hold for Assumption \eqref{bound_norm_non_back} for the glued graphs?
    \item the second assumtion is actually an assumption on the parameter $\epsilon(k)$ as in Lemma \ref{new_graph}. Can we make $k_n$ equal to $m_n$? \ML{In lemma \ref{new_graph} $k$ is arbitrary so I think we can. Also I would like to mention that each of "roots" of the initial graphs can be locally (for some large constant) tree like"}
\end{itemize}




\section{Convergence of growth rate of non-backtracking paths}

\subsection{Settings}
Let $G = (V, E)$ be a locally finite, connected graph. 
Denote by $\text{NB}_{G,u}(n)$ the set of non-backtracking paths of length $n$ in $G$, starting from a vertex $u \in V(G)$. 
Let $\alpha(G) := \lim_{n \rightarrow \infty} |\text{NB}_{G,u}(n)|^{1/n}$. 
Note that this limit does not depend on the initial vertex $u$.
$\alpha$ is the growth rate of the universal cover of $G$. 

\begin{definition}[Non-backtracking matrix]\label{defn_of_non-backtracking}
  Given a locally finite graph $G$, the \emph{non-backtracking matrix} of $G$ is the $|\overrightarrow{E}|\times|\overrightarrow{E}|$ matrix  $B_G$  with entries:
    \[\{B_G\}_{\overrightarrow{e},\overrightarrow{f}}=\mathbf{1}\{\overrightarrow{e}=(u,v) \text{ and } \overrightarrow{f}=(z,w) \text{ such that } v=z \text{ and } u\neq w \}. \]   
    Notice that the dimension of the matrix $B_G$ will be $2 |E(G)|$.
\end{definition}
\begin{definition}
 Let $n \in \N\cup\{\infty\}$ and let a matrix $B$ of dimension $n \times n$. We call the matrix $B$ irrecusible iff for every two indices in $i,j \in[n]$, there exists some $k \in \N$ such that $B^{k}_{i,j}>0$.
\end{definition}

\begin{lemma} \label{lemma:convergence_subgraphs}
    Let $\{G_n\}_{n \in \N}$ be a sequence of finite graphs, such that 
    \begin{enumerate}
        \item $G_n \subseteq G_{n+1}$ and  
        \item $\lim_{n \rightarrow \infty} \alpha(G_n) = \alpha_0$. 
    \end{enumerate}
    Let $G := \cup_{n \in \N} G_n$. Suppose that the degrees of the vertices in $G$ belong all in the set $\{2, \cdots k_{\max}\}$ for some $k_{\max} \in \N$. 
    If $G$ is locally finite and the matrices $B_G$ and $\{B_{G_n}\}_{n \in \N}$ are all irrecusible, then $\alpha(G) = \alpha_0$.
\end{lemma}
\begin{proof}
For any two directed edges in $e,f \in $



    First, since for all $n \in \N$ $G_n \subseteq G$, we have that $\alpha(G) \geq \alpha(G_n)$, thus $\alpha(G) \geq \alpha_0$.

    Let $n \in \N$. 
    By assumption, $\lim_{k\rightarrow \infty}|\text{NB}_{G_n}(k)|^{1/k} = \alpha(G_n)$, so for $k$ large enough, $|\text{NB}_{G_n}(k)| \leq \alpha(G_n)^k + o_k(\alpha(G_n)^k) \leq \alpha(G)^k + o_k(\alpha(G)^k)$, where the last inequity follows from the assumption that $\alpha(G_n) \leq \alpha(G)$.
    
    
    Fix some $u \in G_0$, and let $\text{NB}_G(n) := \text{NB}_{G,u}(n)$. 
    For every $k \in \N$, there exists some $K \in \N$, such that $|\text{NB}_G(k)| \leq |\text{NB}_{G_K}(k)|$, \ML{Shouldn't this be equality?} where $K$ is so that every non-backtracking path of length $k$ does not leave $G_K$.

    Thus, for every $k$ we have 
    \begin{align*} 
        |\text{NB}_{G,u}(k)| \leq |\text{NB}_{G_K,u} (k)| \leq \alpha(G)^k + o_k(\alpha(G)^k) \text{ ,}
    \end{align*}
    so $|\text{NB}_{G,u}(k)|^{1/k} \leq \alpha(G) + \epsilon(k)$, where $\epsilon(k) \rightarrow 0$ as $k \rightarrow \infty$, which concludes the result.

    \ML{Two remarks. Firstly I guess you mean $a_0$ and not $a(G)$ right?. Secondly the bound $NB_{G_n}(k)\leq (a_0+o_k(1))^k$, right? Thus we need to be precise on $o_k(1)$. If for example $o_k(1)=\frac{1}{k},$ then $a_0^k(1+\frac{1}{a_0k})^k\sim (a_0^k \exp(\frac{1}{a_0}))$, which is not what we want. I guess we will be fine if $o_k(1)\sim \frac{1}{k^a}$, for $a>1$.}
\end{proof}

No - the bound is like I wrote, because:
$ (a + \epsilon)$

don't worry about writing more details - do you think the idea is correct? I'll edit it, I just wrote quickly so you can check


